Control Parameters Considered Harmful: Detecting Range Specification Bugs in Drone Configuration Modules via Learning-Guided Search

In order to support a variety of missions and deal with different flight environments, drone control programs typically provide configurable control parameters. However, such a flexibility introduces vulnerabilities. One such vulnerability, referred to as range specification bugs, has been recently identified. The vulnerability originates from the fact that even though each individual parameter receives a value in the recommended value range, certain combinations of parameter values may affect the drone physical stability. In this paper we develop a novel learning-guided search system to find such combinations, that we refer to as incorrect configurations. Our system applies metaheuristic search algorithms mutating configurations to detect the configuration parameters that have values driving the drone to unstable physical states. To guide the mutations, our system leverages a machine learning predictor as the fitness evaluator. Finally, by utilizing multi-objective optimization, our system returns the feasible ranges based on the mutation search results. Because in our system the mutations are guided by a predictor, evaluating the parameter configurations does not require realistic/simulation executions. Therefore, our system supports a comprehensive and yet efficient detection of incorrect configurations. We have carried out an experimental evaluation of our system. The evaluation results show that the system successfully reports potentially incorrect configurations, of which over 85% lead to actual unstable physical states.

==> table/algorithm.tex <==
\begin{algorithm}[ht]
\begin{algorithmic}[1]
\Require  {
Parameter default value($P$), 
Parameter boundary($B$),
Flight model($M$) 
Flight attitude dataset($A$)
}
\Ensure{An unique set of invalid parameters values($Result$)}

\Function{Learning-Guided Mutation Searcher}{$P$,$B$,$M$,$D$}
\State Initialize result set $Result$
\State $A_c \gets \Call{Cluster}{A}$ \Comment{Cluster}
\State $A \gets  \Call{Sampling}{A_c}$ \Comment{Sampling}
\For {$A_t \in A$}
    \State Initialize population $Pop$ according to $P$
    \State Set mutation boundary according to $B$
    \While{evolutionary constraints not satisfied}
        \State $Is \gets \Call{Mutation}{Pop}$ \Comment{Mutation Individual}
        \State $Pop' \gets \Call{Merge}{Pop, Is}$ \Comment{Crossover}
    
        \State $R \gets \Call{Eval}{Pop, M, A_t}$ \Comment{Current population fitness}
        \State $R' \gets \Call{Eval}{Pop', M, A_t}$ \Comment{Experimental population fitness}
        \State $Pop \gets \Call{Update}{Pop, Pop', R, R'}$
    \EndWhile
    \State $Result.\Call{append}{Pop}$
\EndFor
\State $Result \gets \Call{Deduplication}{Result}$
\State \textbf{return} $Result$
\EndFunction 
\Function{Eval}{$Pop, M, A_t$}
    \State $F_{t} \gets \{Pop, A_t\}$ \Comment{Generate feature}
    \State $V_{t+1} \gets\Call{M}{F_{t}}$ \Comment{Predict future states}
    \State $R \gets \Call{CalDeviation}{V_{t+1}}$ \Comment{Calculate fitness}
\State \textbf{return} R
\EndFunction 

\end{algorithmic} 
\caption{Learning-Guided Mutation Searcher.}
\label{alg1}
\end{algorithm}

==> table/feature.tex <==
\begin{table}[ht]
\caption{Construction of fFeature.}
\label{tab:feature}
\centering
\begin{tabular}{c|c}
        \hline
        Feature Class &  Name \\
        \hline
        \hline
        \multirow{6}*{Achieved Attitude} &  1\\
        \cline{2-2}
         ~& INS\_POS2\_Z \\
         \cline{2-2}
         ~& INS\_POS2\_Z \\
         \cline{2-2}
         ~& INS\_POS2\_Z \\
         \cline{2-2}
         ~& INS\_POS2\_Z \\
         \cline{2-2}
         ~& INS\_POS2\_Z \\
        \hline
        \multirow{6}*{Desired Attitude} &  1\\
        \cline{2-2}
         ~& INS\_POS2\_Z \\
         \cline{2-2}
         ~& INS\_POS2\_Z \\
         \cline{2-2}
         ~& INS\_POS2\_Z \\
         \cline{2-2}
         ~& INS\_POS2\_Z \\
         \cline{2-2}
         ~& INS\_POS2\_Z \\
         \hline
        \multirow{1}*{Configuration} &  Attitude-related Control Parameter \\
        \hline
\end{tabular}
\end{table}

==> tex/challenge.tex <==
\siqi{Challenge and solutions are proposed.}

\subsection{Challenges}
\label{sub:challenges}
In order to verify all configurations and detect the invalid ones,
    the following challenges must be addressed: 
    
\vspace{0.15cm}
\noindent
\textbf{Challenge \uppercase\expandafter{\romannumeral1}: How to identify the invalid configurations effectively?}
%and efficiently?}
Approaches proposed for analyzing flight control programs are generally based on static program analysis techniques that explore control and data dependencies~\cite{MAYDAY,Believing,zhu2019new}.
However, 
    such techniques are not suitable for validating configuration
    because a large numbers of specified parameter values need to be analyzed.
Unlike conventional bug detection techniques that statically analyze only small code snippets, 
    the entire flight control program needs to be analyzed in order to achieve a high code coverage. 
The reason is that different parameter values often result in execution flows involving very different portions of the control program. 
Unfortunately, 
    flight control programs have huge sizes (e.g., over 700K lines of code) and complex control and data dependencies,
    %the code included in a flight control program are huge (over 700k lines of code), namely, control and data dependencies are even more complex. 
Therefore, 
    it is critical that the designed approach for configuration validation be effective, 
    that is, 
    able to provide a high coverage of possible parameter values.
% \elisa{below you say that the approach has to be effective and efficient. Effective basically means that it can find all the invalid configuration. What do you mean by "efficient"? I was thinking that we could remove the efficiency from this challenge as it is addressed by next challenge. If you agree, we can change the title of this challenge and focus the challenge on the effectiveness.}
% and efficient.
%
    
%%%%%%%%%%%% Rain Raw %%%%%%%%%%%%%%%%%
%The unreasonable range implement is caused by the system logic design, 
%    but considering the huge number of configuration parameters, 
%    it is complicated to do code-level static analysis for each parameter,
%   that requires tremendous data flow and parameter correlation analysis.
%And even many configurations do not exhibit system-level symptoms until certain control and physical conditions are met at run-time.

    
% 对configuration的每一次验证消耗巨大，一个一个的测十分费时，效率不高
\vspace{0.15cm}
\noindent
\textbf{Challenge \uppercase\expandafter{\romannumeral2}: How to conduct an efficient configuration validation?
%reduce the unnecessary verification bottleneck in search?
}
Referring to the unstable flight states defined in Section~\ref{sec:back}, 
    we need to validate the correctness of each configuration through either a 
    % \elisa{what do you mean by "real execution"? do you mean by a real flight?}
    \rain{realistic or simulated flight execution}. 
However, 
    testing the correctness of all configurations by combining all potential parameter values is inefficient. 
As we need to consider multiple parameters, each with its own value range, multiple value ranges will have to be verified. 
%When multiple parameters are considered, more value ranges need to be verified; 
%Thus the searching range would increase exponentially. 
%It may then require hours
Completing the entire validation procedure may then end up requiring hours. 
Therefore, existing approaches~\cite{tartler,halin2019test} that analyze all possible configurations are not suitable.
%targeting on analyzing all configuration. 
    
Instead of verifying all possible configurations, an approach is to use fuzzing~\cite{rvfuzzer} combined with binary search~\cite{knuth1971optimum} to reduce the search space of the combinations to be analyzed.
%Consider \tool{RVFUZZER}~\cite{rvfuzzer} as an example, %it combines fuzzing with the binary search algorithm to neglect unnecessary searches. 
However, although search scope is narrowed, the execution cost increases because each fuzzing iteration needs to wait until the validation feedback of the previous configuration is obtained.
%Hence an efficient approach that could not only constraint the search scope, 
%but also decrease the execution cost is preferred. 
   
%%%%%%%%%%%% Rain Raw %%%%%%%%%%%%%%%%%
%The validity of a configuration needs to be verified by either actual or simulator execution,
%    which becomes the bottleneck of search.
%Even if the clock speed simulator is used, 
%    execution verification still takes nearly ten seconds for one value.    
%And a parameter often has multiple optional values (e.g., \param{ATC\_RAT\_PIT\_I} has $98$). 
%Thus,
%    directly verifying each value will consume a huge amount of resources. 
%Previous research \rvfuzzing leverages binary search algorithms to skip search space for reducing unnecessary execution.
%However,
%    as binary search is seek-feedback-seek form (next search target needs the previous feedback),
%    \rvfuzzing search efficiency is still limited,
%    where the time consumed for execution is much larger than the time consumed for one search.



%%%%%%%%%%%% Rain Raw %%%%%%%%%%%%%%%%%。
%\noindent
%\textbf{Challenge II: How to search for the parameters causing invalid configurations?}
%effectively solve a broad space search among multi-parameter problems?}
%In order to search for the 
%Give value ranges of parameters, 
%    it is inefficient to test all configurations by combining every parameter value. 
    
    
%The difficulty of searching multi-parameter invalid configurations increases exponentially with the increase of the number of parameters,
%    that is even more impossible to use coverage to test every configuration.
%In addition,
%    the multi-parameter have more mutation direction,
%    which also increases the difficulty of the search direction decision.
%Therefore, 
%    it is important to adopt an efficient search method that can skip unnecessary search space and provide more suitable mutations direction.
 


\vspace{0.15cm}
\noindent
\textbf{Challenge \uppercase\expandafter{\romannumeral3}: How to balance the requirement of \rain{adaptability and stability}?}
% flight stability and scalability?}
The flight control program supports different configurations to adapt to different flight missions. 
%\elisa{I would not use the term "scalability" here. I would say something like "In order to enhance adaptability to different missions, parameter value ranges indicated by the manufacturers are quite wide." I would also title the the challenge as "How to balance adaptability and stability" }
When high \rain{adaptability} is provided, 
    each parameter must have a large value range 
    %of each parameter has to large 
    to adapt to different scenarios.
    As a result, the number of invalid configurations will be higher, which will then affect flight stability.
%It indicates that more invalid configurations will be included, that is, flight stability will be low. 
On the other hand, when parameters have small value ranges, the possible configurations are limited, which reduces adaptability. As a consequence, complex flight missions cannot be carried out.
    %when limited configurations (i.e., small value range of each parameter) are provided, 
    %flight scalability will be affected; thus complex flight mission may not be achieved. 
Identifying proper value ranges is thus challenging.
   % it is difficult for us to provide an appropriate suggestion of value range selection to users and developers.
    
%The essence of providing a reasonable range is to eliminate invalid configuration points in the range. 
%However, 
%    although the too narrow range improves the security, 
%    it reduces the choice of customer,
%    that some invalid configurations cause instability only under extreme conditions. 
%Normally, 
%    non-professional customers lack the knowledge to set up a reasonable configuration to balance security and availability.
    
\subsection{Solutions}
\label{sub:solution}
We now introduce our approaches to those challenges.
%address the challenges discussed in the previous section.
%For each challenge introduced in Section~\ref{sub:challenges}, we proposed three approaches to address them respectively. 
    
\vspace{0.15cm}
\noindent
\textbf{Solution I: Grey-box based fuzzing.}
Since dependencies of  flight control programs are complex, static program analysis techniques are ineffective.
   % it is ineffective and inefficient to conduct static program analysis. 
Our approach is instead to  
    %we aim 
conduct grey-box based fuzzing by setting various configurations and verifying the corresponding flight states. 
In particular, we first apply a
    %we execute the 
    genetic algorithm to select a valid value for each parameter; then the resulting parameter configuration is validated. Validation of the configuration is performed by analyzing its impact on the flight states.
    %and take the configuration as input for validation. 
Through the mutation search, 
    the invalid configurations 
    %(i.e., causing incorrect configurations) 
    are discarded.
   % (i.e., configurations that are not acceptable by flight control systems) will be neglected.
%Then we distinguish configurations by examining its impact to the flight states, %that is, any configurations causing unstable flight states are invalid.
This approach addresses challenges I and II. 

%Instead of static code analysis,
%    we make use of a grey-box fuzzing with genetic algorithm to search the invalid configurations.
%This multi-dimensional mutation search can effectively deal with multi-parameter search problems,
%    that accurately determines the mutation direction to skip the useless search space. 
%The genetic algorithm based fuzzing simultaneously solves the problems of search methods and multi-parameter broad space. 

\vspace{0.15cm}
\noindent
\textbf{Solution II: Flight state prediction}
%Learning based fitness function.}
\elisa{this is a bit confusing, I was under the impression that also the genetic algorithm needs the feedback}
Fuzzing requires state feedback about the previous configuration before the next iteration and such configuration validation requires to fly realistic drones or execute simulators, 
    which takes several seconds to obtain the state feedback.
    % \elisa{I'm not sure about the remark below. Nobody would indeed think that genetic algorithm would help here as the task of the genetic algorithm is not to fly the drone or simulate the flight. I have thus commented out the sentence below.}
%Therefore, only relying on the genetic algorithm is in efficient. 
In response, 
    we designed a state generation approach, 
    which generates a prediction model by leveraging a machine learning algorithm and further takes the configuration as input to predict the potential flight state for \rain{mutation guide}. 
Model prediction takes much less than flying a real drone or executing the drone simulation. 
Noted that data labeling and model training are only one-time cost; hence it is more efficient to conduct model prediction rather than reality execution iteratively.
This solution addresses Challenge II.


%To reduce the execution verification bottleneck,
%    we use a learning model prediction instead of the execution as feedback of genetic algorithm,
%    which model predictions take much less time than execution.
%This alternative can put time-consuming execution verification after the search. 
%The search only needs to find those potential configurations that model considers have a high probability to cause instability events. 
%Finally,
%    we can concurrently verify potential configurations to find the invalid configurations.

\vspace{0.15cm}
\noindent
\textbf{Solution III: Multi-objective optimization.}
\elisa{the text below does not really say much about how to balance adaptability and stability. It just mention that there are security levels and that they are different for different types of missions. The text does not say what the security levels are; are they some numbers?. The text needs to be better connected to the challenge III}
We propose a multi-objective optimization approach
\elisa{do you mean that the multi-objective optimization takes as input a security level and finds the optimal parameter configuration?}
with variant security levels. 
Referring to the purpose of flying drones (e.g., photo shooting for commercial usage, surveillance for military), 
    the corresponding security requirements are different. 
According to the security requirement
    our approach will provide the different range of parameter values.
For instance, 
    drones for military surveillance are typically given a small value range for each parameter because it is critical that the drone flight to be stable. 
This approach addresses Challenge III. 
    
    
%When invalid configurations are found out,
%    to balance security and availability,
%    we leverages the multi-objective optimization to summarize feasible ranges that attempt to avoid those invalid configurations and fully utilize the verification.



